Improving IoT Analytics through Selective Edge Execution

A large number of emerging IoT applications rely on machine learning routines for analyzing data. Executing such tasks at the user devices improves response time and economizes network resources. However, due to power and computing limitations, the devices often cannot support such resource-intensive routines and fail to accurately execute the analytics. In this work, we propose to improve the performance of analytics by leveraging edge infrastructure. We devise an algorithm that enables the IoT devices to execute their routines locally; and then outsource them to cloudlet servers, only if they predict they will gain a significant performance improvement. It uses an approximate dual subgradient method, making minimal assumptions about the statistical properties of the system's parameters. Our analysis demonstrates that our proposed algorithm can intelligently leverage the cloudlet, adapting to the service requirements.

==> Extensions_V4.tex <==
\section{Model and Algorithm Extensions} \label{sec:extensions}

Our framework can be used in different systems and types of tasks. In this section we extend it for multiple cloudlets where the devices can select \emph{where} to outsource their tasks. Then, we explain how it can cope with massive demand scenarios, where the wireless bandwidth becomes a constraint; and finally we elaborate on alternative designs/usages of the predictor.% and discuss how it can reduce energy consumption by making outsourcing decisions without local classifications.
 

\textbf{Multiple Cloudlets}: We denote with $k=1, 2, \ldots, K$ the cloudlets, which have computing capacity $\{H_{kt}\}_{t=1}^{\infty}$. Each device $n$ has a different predictor for each cloudlet. The decision of device $n$ will be given by $x_{nkt}\in\{0,1\}$ that determines if cloudlet $k$ will be used with expected improvement $w_{nkt}$. The constraint $\sum_{k=1}^{K}x_{nkt}\leq 1, \forall n, t$ should be added, and this changes the set of possible values for $x_{nkt}$ in each slot. The respective static continuous problem here is:
\begin{align}
\text{(P2-K)}:\qquad&\min_{y_{nk}^j\in[0,1], \forall n,k,j} -\sum_{j=1}^{M}\sum_{n=1}^N\sum_{k=1}^{K} w_{nk}^j\lambda_{nk}^jy_{nk}^j\\
	\text{s.t.}\,\qquad	&\sum_{j=1}^{M}\sum_{k=1}^K y_{nk}^j\lambda_{nk}^jo_{n} \le B_{n},\,n\in\mathcal{N},\label{eq:P1K-device-constraintb}\\
	&\sum_{m=1}^M\sum_{n=1}^Ny_{nk}^j\lambda_{nk}^jh_{nk} \le H_{k},\forall k\in\mathcal{K} \label{eq:P1K-cloudlet-constraintb},\\
	&\sum_{k=1}^Ky_{nk}^j \le 1,\,\,\forall n\in\mathcal{N}, \forall j\,. \label{eq:P1K-time-constraintb}
\end{align}
Note that this extension essentially only increases the problem's dimension, and adds constraint \eqref{eq:P1K-time-constraintb} which needs to be satisfied in each slot. The Lagrangian can be defined as $L(\bm y, \bm \mu)=$
\begin{align}
- \sum_{j=1}^M\sum_{n=1}^N\sum_{k=1}^K w_{nk}^j y_{nk}^j \lambda_{nk}^j + \sum_{n=1}^{N}\mu_n\Big( \sum_{k=1}^K\sum_{j=1}^Mo_n\lambda_{nk}^jy_{nk}^j-B_n \Big)+\sum_{k=1}^K \xi_k\Big( \sum_{j=1}^M\sum_{n=1}^Ny_{nk}^j\lambda_{nk}^jh_{nk}-H_k \Big). \nonumber
\end{align}
The primal update will employ the following simple rule (for the complete information):
\begin{align}
	\big( y_{nk}^j\big)^*= \argmin_{y_{nk}^j\in [0,1] } \{y_{nk}^j\big( -w_{nk}^j \!+\! \mu_no_n \!+\! \xi_kh_{nk}\big),\,\, \forall k\}. \nonumber
\end{align}
This expression yields a \emph{bang-bang} policy and hence maximizes the Lagrangian while satisfying \eqref{eq:P1K-time-constraintb}. The dual updates are trivial extensions of the ones in the single-cloudlet scenario. %This extension affects the convergence of the algorithm, but only through the constant factors. 

\textbf{Wireless Bandwidth Constraints}: We have assumed the system operation is constrained by the devices' power budget and the computing capacity of the cloudlet. Indeed, most often these are the bottleneck resources \cite{Cloudlets,letaief-edge-tutorial,Smart_cities}. However, in scenarios of massive demand the wireless link capacity might also be a bottleneck constraint. Our analysis can be readily extended for this case. If we denote with $\{W_t\}_{t=1}^{\infty}$ the link capacity process (uniformly bounded; well-defined mean value) assuming a wireless link shared by all devices\footnote{This can be either an OFDM-based cellular link or a coordinated access WiFi link; in the case we have a CSMA-type of mechanism, one needs to account for the additional bandwidth loss due to collisions, etc.}, we can add to (P1) the constraint:
\begin{equation}
	\lim_{T\rightarrow \infty}\frac{1}{T}\sum_{n=1}^N\sum_{t=1}^T\sum_{j=1}^M x_{nt}^j\lambda_{nt}^j\ell_{n} \leq	\lim_{T\rightarrow \infty}\frac{1}{T}\sum_{t=1}^TW_t , \label{eq:link-constraint-new}
\end{equation}
where $\ell_{n}$ is the size of objects (in MBytes) device $n$ transmits. Eq. \eqref{eq:link-constraint-new} can be handled as the computing constraint \eqref{eq:P1-cloudlet-constraint}, and will only affect the convergence bounds. Similarly, we can include other constraints, coupling the actions of all devices $\forall t$, or separately of each device across time.


\textbf{Predictors and Multi-stage Tasks}: A different mechanism is possible, where the devices send objects to the cloudlet before using their own classifier. This approach can reduce the consumed energy, since it avoids low-accuracy local classifications. However, it requires a different type of a predictor, namely one that can estimate the expected accuracy gain using some basic features of the object (e.g., its file size), and without requiring input from the local classifier. The OnAlgo algorithm can be extended to this case by changing the predictor, as long as Assumption 1 holds. 

Similarly, it is possible to have analytic services that are executed in multiple stages, e.g., a video stream is compressed, then frames of interest are selected, and objects of are identified on each frame. In this case, the devices might decide to outsource some of the tasks in the first stage, some others after the second stage, and so on. Again, our optimization algorithms can be extended to include these decisions, by defining a separate set of variables for each stage while accounting for the costs and properties (e.g., data volumes) in each case.

%-- transmit without local classification

%-- transmit only the extracted features
